Robust Constrained Reinforcement Learning for Continuous Control with Model Misspecification

Many real-world physical control systems are required to satisfy constraints upon deployment. Furthermore, real-world systems are often subject to effects such as non-stationarity, wear-and-tear, uncalibrated sensors and so on. Such effects effectively perturb the system dynamics and can cause a policy trained successfully in one domain to perform poorly when deployed to a perturbed version of the same domain. This can affect a policy's ability to maximize future rewards as well as the extent to which it satisfies constraints. We refer to this as constrained model misspecification. We present an algorithm that mitigates this form of misspecification, and showcase its performance in multiple simulated Mujoco tasks from the Real World Reinforcement Learning (RWRL) suite.

==> defs.tex <==
% Citing
\newcommand{\cp}{\citep}
\newcommand{\ca}{\citeauthor}
\newcommand{\cy}{\citeyear}
\newcommand{\ct}{\citet}
\newcommand{\ctp}[1]{\ca{#1}'s~(\cy{#1})}
\newcommand{\cwp}[1]{\ca{#1}, \cy{#1}}
\newcommand{\ctt}[1]{\ca{#1}~\cp{#1}} % this is to avoid [] in the next line

\newcommand{\mat}[1]{\ensuremath{\boldsymbol{\mathrm{#1}}}}
\newcommand{\fnc}[1]{\ensuremath{\mathrm{#1}}}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}

\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\M}{\ensuremath{\mathcal{M}^{\phi}}}
\newcommand{\MM}{\ensuremath{\mathcal{M}}} 
\newcommand{\CC}{\ensuremath{\mathcal{C}}} 
\newcommand{\E}{\ensuremath{\mathrm{E}}}
\newcommand{\MMtr}{\ensuremath{\hat{\MM}}} 
\newcommand{\Mtr}{\ensuremath{\hat{M}}}
\newcommand{\wtr}{\ensuremath{\hat{\mat{w}}}}
\newcommand{\rtr}{\ensuremath{\hat{r}}}
\newcommand{\rvtr}{\ensuremath{\hat{\mat{r}}}}
\newcommand{\Rtr}{\ensuremath{\hat{R}}}
\newcommand{\Wtr}{\ensuremath{\hat{\mat{W}}}}

\newcommand{\Normal}{\ensuremath{\mathcal{N}}}

\newcommand{\w}{\mat{w}}
\newcommand{\WW}{\mat{W}}
\newcommand{\Wt}{\ensuremath{\tilde{\mat{W}}}}
\renewcommand{\r}{\mat{r}}
\newcommand{\z}{\mat{z}}
\newcommand{\zw}{\mat{zw}}
\newcommand{\Z}{\mat{Z}}
\newcommand{\vphi}{\mat{\phi}}
\newcommand{\vpsi}{\mat{\psi}}
\newcommand{\vprm}{\mat{\z}}
\newcommand{\tvphi}{\ensuremath{\tilde{\mat{\phi}}}}
\newcommand{\tvpsi}{\ensuremath{\tilde{\mat{\psi}} }}
\newcommand{\tPsi}{\ensuremath{\tilde{\Psi} }}
\newcommand{\tmpsi}{\ensuremath{\tilde{\mat{\Psi}} }}
\newcommand{\MPhi}{\mat{\Phi}}
\newcommand{\MPsi}{\mat{\Psi}}
\renewcommand{\P}{\mat{P}}
\renewcommand{\t}{\ensuremath{\top}}



\renewcommand{\th}[1]{\text{#1$^\mathrm{th}$}}
\newcommand{\ith}{\th{i}}
\newcommand{\jth}{\th{j}}
\newcommand{\kth}{\th{k}}

\newcommand{\argmin}{\ensuremath{\mathrm{argmin}}}
\newcommand{\argmax}{\ensuremath{\mathrm{argmax}}}
\renewcommand{\min}{\ensuremath{\mathrm{min}}}

\newcommand{\Qmax}{\ensuremath{Q_{\mathrm{max}}}}
\newcommand{\pimax}{\ensuremath{\pi_{\max}}}
\newcommand{\Qpimax}{\ensuremath{Q^{\pi_{\max}}}}
\newcommand{\Tpimax}{\ensuremath{T^{\pi_{\max}}}}

\newcommand{\Mh}{\ensuremath{\hat{M}}} 
\newcommand{\Qh}{\ensuremath{\hat{Q}}}
\newcommand{\pih}{\ensuremath{\hat{\pi}}}
\newcommand{\wh}{\ensuremath{\hat{\w}}}
\newcommand{\Qhmax}{\ensuremath{\hat{Q}_{\mathrm{max}}}}
\newcommand{\pihmax}{\ensuremath{\pi}}
\newcommand{\Qhpimax}{\ensuremath{\hat{Q}^{\pi_{\max}}}}
\newcommand{\Thpimax}{\ensuremath{\hat{T}^{\pi_{\max}}}}

\newcommand{\rdif}{\ensuremath{\delta}}

\newcommand{\Qt}{\ensuremath{\tilde{Q}}}
\newcommand{\vQt}{\ensuremath{\tilde{\mat{Q}}}}
\newcommand{\pit}{\ensuremath{\tilde{\pi}}}
\newcommand{\Qtmax}{\ensuremath{\tilde{Q}_{\mathrm{max}}}}
\newcommand{\pitmax}{\ensuremath{{\pi}}}
\newcommand{\Qpitmax}{\ensuremath{Q^{\pi}}}
\newcommand{\Tpitmax}{\ensuremath{T^{\pi}}}
\newcommand{\wt}{\ensuremath{\tilde{\w}}}
\renewcommand{\H}{\mat{H}} 

\newcommand{\agt}{\fnc{agt}}

\newcommand{\piexp}{\ensuremath{\pi}}
\newcommand{\piexpj}{\ensuremath{_{\piexp_j}}}
\newcommand{\piexpi}{\ensuremath{_{\piexp_i}}}
\newcommand{\piexpk}{\ensuremath{_{\piexp_k}}}

\newcommand{\la}{\ensuremath{\leftarrow}}

\newcommand{\vpi}{\ensuremath{\mat{v}^{\pi}}}
\newcommand{\rpi}{\ensuremath{\mat{r}^{\pi}}}
\newcommand{\Ppi}{\ensuremath{\mat{P}^{\pi}}}

\newcommand{\phimax}{\ensuremath{\vphi_{\max}}}

\renewcommand{\S}{\ensuremath{\mathcal{S}}}
\newcommand{\A}{\ensuremath{\mathcal{A}}}
\newcommand{\W}{\ensuremath{\mathcal{W}}}

\newcommand{\score}{\ensuremath{\mathrm{score}}}
\newcommand{\currscore}{\ensuremath{\mathrm{curr\_score}}}
\newcommand{\ntpu}{\ensuremath{\mathrm{used}}}
\newcommand{\act}{\ensuremath{\mathrm{c}}}

\newcommand{\I}[1]{\ensuremath{\delta\{#1\}}} 
\newcommand{\II}{\ensuremath{\delta}} 

\newcommand{\vf}{\ensuremath{\mat{\varphi}}}
\newcommand{\vfi}{\ensuremath{\mat{\varphi}_i}}
\newcommand{\vfp}{\ensuremath{\mat{\varphi}_p}}
\newcommand{\vweights}{\mat{z}}
\newcommand{\od}{\ensuremath{\mat{o}}}
\newcommand{\rank}{\ensuremath{\mathrm{rank}}}

\newcommand{\ns}{\ensuremath{\mathrm{ns}}}
\newcommand{\nstr}{\ensuremath{n_{\mathrm{tr}}}}
\newcommand{\nsts}{\ensuremath{n_{\mathrm{ts}}}}
\newcommand{\dist}{\ensuremath{\mathcal{D}}}
\newcommand{\rt}{\ensuremath{\tilde{r}}}
\newcommand{\rvt}{\ensuremath{\tilde{\mat{r}}}}
\newcommand{\vrt}{\ensuremath{\tilde{\mat{r}}}}
\newcommand{\params}{\ensuremath{\mat{\theta}}}

\newcommand{\eb}{\ensuremath{\mathrm{extend\_basis}}}
\newcommand{\sfgpi}{SF\hspace{0.2mm}\&\hspace{0.2mm}GPI}
\newcommand{\sfgpirl}{\sfgpi\ continual}
\newcommand{\sfgpisl}{\sfgpi\ zero-shot}

\newcommand{\mo}{{\normalfont-{\tt 1}}}
\newcommand{\taskfive}{{\tt 1100}}
\newcommand{\tasksix}{{\tt 0111}}
\newcommand{\taskseven}{{\tt 1111}}
\newcommand{\taskeight}{{\tt \mo000}}
\newcommand{\tasknine}{{\tt \mo\mo00}}
\newcommand{\taskten}{{\tt \mo100}}
\newcommand{\taskeleven}{{\tt \mo1\mo0}}
\newcommand{\tasktwelve}{{\tt \mo101}}
\newcommand{\taskthirteen}{{\tt \mo1\mo1}}
\newcommand{\taskexample}{{\tt 1\mo00}}


\newcommand{\pitest}{\ensuremath{\pi_{\mathrm{test}}}}

\renewcommand{\dist}{\ensuremath{\mathcal{D}}}

\newcommand{\tderrorz}{\ensuremath{\mat{\delta}_{\z}^{t,n}}}
\newcommand{\tderrorwz}{\ensuremath{\mat{\delta}_{\w\z}^{t,n}}}

==> old_intro.tex <==
% By incorporating robustness into our agents, we correct for this misspecification yielding improved performance in the perturbed environment(s). \cosmo{What is the type of real-world scenario we should have in mind for this? Sim2Real? Something else?}



% , an increasing number of high impact applications such as autonomous driving and building control systems are starting to utilize deep learning to make crucial real-time decisions. In these systems, making the wrong decision, (e.g., Incorrectly classifying a stop-sign in an autonomous driving system) can have serious consequences, which further motivates the need for these systems to be robust.



% \textbf{TL;DR: This is a rough draft of what a paper might look like for RL with verification. Comments and feedback welcome.}

% \cosmo{Cool! My general comment on the intro is that it would be good to make it clearer that this aims to solve the problem of constrained RL in the presence of (adversarial) perturbations, but I am sure we can get there over time.}

% However,the field of Reinforcement Learning (RL) \citep{sutton2018reinforcement} has not as yet realized the full benefits of this adversarial/verifiable training regime. This is due to a number of different challenges that still need to be solved such as: (1) Defining the adversarial/verifiable RL objective; (2) providing theoretical guarantees for this objective and (3) developing algorithmic solutions to optimize this objective. \cosmo{Probably useful to specify different potential types of perturbations - e.g. input perturbations, action perturbations, reward perturbations, dynamics perturbations, and discuss which one(s) this paper is addressing. Is it just dynamics, as the paragraph below might indicate?}

% \textbf{Model misspecification}: For the purpose of this paper, we refer to an agent that is trained in one environment and performs poorly, with respect to constraint satisfaction, in a different, perturbed version of the environment (as in the above examples) as \textit{model misspecification}. By incorporating robustness into our agents, we correct for this misspecification yielding improved performance in the perturbed environment(s). \cosmo{What is the type of real-world scenario we should have in mind for this? Sim2Real? Something else?}

% In addition, many of these systems have constraints that need to be adhered to upon deployment. If constraints are not satisfied.....\textbf{TODO}

%What is the problem?
% It is well-known that neural networks are not robust \citep{goodfellow_deep_2016}. It has been shown that adding carefully selected deviations to the input, which are referred to as adversarial perturbations, can cause the networks to make incorrect predictions with high confidence \citep{carlini_adversarial_2017,carlini_towards_2017,goodfellow_explaining_2014,kurakin_adversarial_2016,szegedy_intriguing_2013}.  


% Much work has been done in the deep learning community towards training neural networks to being robust to adversarial perturbations  \citep{goodfellow_explaining_2014,papernot_distillation_2015,madry_towards_2017,kannan_adversarial_2018,xie_feature_2018}. \danm{Discuss verification and adversarial training in more detail.}\cosmo{Would be great to also have some examples that are not just research but used in some production system (not sure if any of these already are?).}
\textbf{Main Contributions:} In this paper we have the following contributions:

\begin{itemize}
    \item Adapting MPO to handle constraints (MPO-L)
    \item Adapt MPO-L to handle robustness to state perturbations (MPO-LR)
    \item Adapt the robust RL objective to handle constraints with theoretical guarantees of convergences (Robust Constrained RL objective)
    \item Show that a variation of this objective that is robust with respect to constraints only is an (upper bound?) to the above objective - show the connection to verification
    \item MPO-LR, SVG-LR and show that they are robust to model misspecification on \textbf{four} Mujoco domains
    \item Connect the multi-headed MPO-LR, SVG-LR to the above objective - apply different techniques (possible IBP-style, simple worst case) for solving the optimization with respect to the constraint value function prediction 
    \item Baselines:
    % MPO, MPO-R, MPO-LR, MPO-L, SVG...
    \item Propose a verifiable constrained RL objective and  show that this is a special case of the Robust RL objective.
    \item Provide theoretical guarantees for this objective.
    \item Incorporate verification/adversarial training techniques into Maximum a-Posteriori Policy Optimization  \citep{abdolmaleki2018maximum} and Stochastic Value Gradients \citep{heess2015learning} and show that these algorithms are able to satisfy constraints and are robust to model misspecification on \textbf{four} Mujoco domains. We refer to the variants as Verifiable Constrained MPO (VC-MPO) and Verifiable Constrained SVG (VC-SVG).
\end{itemize}

==> old_proof.tex <==

% \begin{eqnarray}
%     \max_{\pi \in \Pi} \min_{p\in P} \mathbb{E}^{P, \pi}\biggl[\sum_t \gamma^t r(s_t,a_t) \biggr]&&\\
%     \text{s.t.} \forall s_t \in S, a_t \sim \pi, \mathbb{E}\biggl[\sum \gamma c(s_t,a_t) < \beta
% \end{eqnarray}

% \begin{eqnarray}
%     \max_{\pi \in \Pi} \min_{p\in P} \mathbb{E}^{P, \pi}\biggl[\sum_t \gamma^t (r(s_t,a_t) - \lambda (c(s_t,a_t)-\beta)) \biggr]&&\\
%     \max_{\pi \in \Pi} \min_{p\in P} \mathbb{E}^{P, \pi}\biggl[V_R - \lambda (V_C-\beta*\frac{1}{(1-\gamma)}) \biggr]&&\\
%      \max_{\pi \in \Pi} \min_{p\in P} \mathbb{E}^{P, \pi}[V_R] - \lambda \min_{p\in P} \mathbb{E}^{P, \pi}[V_C-\beta*\frac{1}{(1-\gamma)}]&&\\
%      ?? \max_{\pi \in \Pi}\biggl[ [V_R] - \lambda \min_{p\in P} \mathbb{E}^{P, \pi}[V_C] ]\biggr]&&\\
%      ?? \max_{\pi \in \Pi}\biggl[ [V_R] - \lambda \min_{p\in P} \mathbb{E}^{P, \pi}[V_C-\beta] ]\biggr]&&\\
% \end{eqnarray}


This can be equally defined as a combination of two separate Bellman operators. That is, 

\begin{equation}
    T^\pi \tilde{V} = T^\pi_{\rm inf} V - \lambda T^\pi_{\rm sup} V_C
\end{equation}

We refer to the operator $T^\pi_{\rm inf}:\mathbb{R}^d \rightarrow \mathbb{R}^d$ as the robust Bellman operator:

\begin{equation}
    T^\pi_{\rm inf} V = r(s,\pi(s)) + \gamma \biggl[ \inf_{p \in P} \mathbb{E}^{P, \pi} \biggl(V(s') \biggr) \biggr]
\end{equation}

We know from previous work that this Bellman operator is a contraction based on the proofs from \citep{tamar2014scaling,iyengar2005robust}. The second operator we refer to as the robust constrained Bellman operator $T^\pi_{\rm sup}:\mathbb{R}^d \rightarrow \mathbb{R}^d$:

\begin{equation}
    T^\pi_{\rm sup} V_c = c(s,\pi(s)) + \gamma  \biggl[ \sup_{p \in P} \mathbb{E}^{P, \pi} \biggl( V_c(s') \biggr) \biggr] - \beta 
\end{equation}

\begin{customthm}{Joint Robust Bellman operator}
For two arbitrary value functions $U:S\rightarrow \mathbb{R}^d$ and $V:S\rightarrow \mathbb{R}^d$, we can show that the robust constrained Bellman operator $\mathcal{T}^{\pi}:\mathbb{R}^d \rightarrow \mathbb{R}^d$ is a contraction. That is 

\begin{equation}
\Vert \mathcal{T}^{\pi} \tilde{U}(s) - \mathcal{T}^{\pi} \tilde{V}(s) \Vert_\infty \leq \gamma \Vert \tilde{U} - \tilde{V} \Vert_\infty
\end{equation}
\end{customthm}

\begin{proof}
Now, to show that this Bellman operator is a contraction, we can do the following:
\begin{align*}
    \| T^\pi \tilde{V} - T^\pi \tilde{U} \|_\infty &= \| (T^\pi_{\rm inf} V - \lambda T^\pi_{\rm sup} V_C) - (T^\pi_{\rm inf} U - \lambda T^\pi_{\rm sup} U_C) \|_\infty \\
    &= \| (T^\pi_{\rm inf} V -  T^\pi_{\rm inf} U) + \lambda (T^\pi_{\rm sup} U_C - T^\pi_{\rm sup} V_C) \|_\infty \\
    &\leq \| T^\pi_{\rm inf} V -  T^\pi_{\rm inf} U \|_\infty + \| \lambda (T^\pi_{\rm sup} U_C - T^\pi_{\rm sup} V_C) \|_\infty && \textrm{By subadditivity of $\|\cdot\|_\infty$.} \\
    &\leq \underbrace{\| T^\pi_{\rm inf} V -  T^\pi_{\rm inf} U \|_\infty}_{(a)} + \lambda \cdot \underbrace{\| T^\pi_{\rm sup} U_C - T^\pi_{\rm sup} V_C \|_\infty}_{(b)} && \textrm{By absolute scalability of $\|\cdot\|_\infty$ and $\lambda \geq 0$.}
\end{align*}

Since $(a)$ is already a contraction based on the proofs from \citep{tamar2014scaling,iyengar2005robust}, we only need to prove that $(b)$ is a contraction. It seems like we might even be able to use the same arguments to show that $(b)$ is a contraction.

\end{proof}


Now, to show that this Bellman operator is a contraction, we can do the following:

\begin{proof}
We follow the proofs from \citep{tamar2014scaling,iyengar2005robust}, Let $\tilde{U},\tilde{V} \in \mathbb{R}^{|S|}$, and $s \in S$ an arbitrary state. Assume $\mathcal{T}^{\pi} \tilde{U}(s) \geq \mathcal{T}^\pi \tilde{V}(s)$. Let $\epsilon > 0$ be an arbitrary positive number. 

By the definition of the $\inf$ operator, there exists $p_{s} \in \mathcal{P}$ such that,

\begin{multline}
    r(s, a) - \lambda c(s,a) + \gamma \mathbb{E}_{s' \sim p_{s}(\cdot|s,a)} V(s') - \lambda \gamma \mathbb{E}_{s' \sim p_{s}(\cdot|s,a)} V_C(s') + \lambda \beta \\
    <  r(s, a) - \lambda c(s,a) + \gamma \inf_{p \in \mathcal{P}} \mathbb{E}_{a \sim \pi(\cdot |s)}V(s') -\lambda \gamma \sup_{p \in \mathcal{P}} \mathbb{E}_{a \sim \pi(\cdot |s)}V_C(s') + \lambda \beta + \epsilon    
\end{multline}


In addition, we have by definition that:
% \kingtim{Is the $p_s$ used in the following equation the same as the $p_s$ in the equation above? Or are these two separate elements?}
% \danm{It is the same one.}
\begin{multline}
    r(s, a) - \lambda c(s,a) + \gamma \mathbb{E}_{s' \sim p_{s}(\cdot|s,a)} U(s') -\lambda \gamma \mathbb{E}_{s' \sim p_{s}(\cdot|s,a)} U_C(s') + \lambda \beta \\
    \geq  r(s, a) - \lambda c(s,a) + \gamma \inf_{p \in \mathcal{P}} \mathbb{E}_{a \sim \pi(\cdot |s)} U(s') - \lambda \gamma \sup_{p \in \mathcal{P}} \mathbb{E}_{a \sim \pi(\cdot |s)} V_C(s') +\lambda \beta
\end{multline}

Thus, we have,

\begin{equation}
\begin{split}
0 &\leq \mathcal{T}^{\pi} \tilde{U}(s) - \mathcal{T}^{\pi} \tilde{V}(s)\\
&<   r(s, a) - \lambda c(s,a) + \gamma \mathbb{E}_{s' \sim p_{s}(\cdot|s,a)} U(s') -\lambda \gamma \mathbb{E}_{s' \sim p_{s}(\cdot|s,a)} U_C(s') + \lambda \beta\\
& \quad - [r(s, a) - \lambda c(s,a) + \gamma \mathbb{E}_{s' \sim p_{s}(\cdot|s,a)} V(s') - \lambda \gamma \mathbb{E}_{s' \sim p_{s}(\cdot|s,a)} V_C(s') + \lambda \beta] + \epsilon\\
&= \mathbb{E}_{a \sim \pi(\cdot |s), s' \sim p_s(\cdot|s,a)} [ \gamma U(s')] - \lambda \mathbb{E}_{a \sim \pi(\cdot |s), s' \sim p_s(\cdot|s,a)} [ \gamma U_C(s')] \\
& \quad - \mathbb{E}_{a \sim \pi(\cdot |s), s' \sim p_s(\cdot|s,a)} [ \gamma V(s')] + \lambda \mathbb{E}_{a \sim \pi(\cdot |s), s' \sim p_s(\cdot|s,a)} [ \gamma V_C(s')]+ \epsilon\\
& \leq \gamma \Vert U - V \Vert_\infty - \lambda \Vert U_C - V_C \Vert_\infty\\
& \leq \gamma \Vert U - V \Vert_\infty\\
%&\leq \gamma \Vert U - V \Vert + \epsilon
\end{split}
\end{equation}
\textbf{To do... Can we set $\tilde{V}=V - \lambda V_C$ and get a constraction with respect to $\tilde{V}$?}

\textbf{To do... Still need to get to the step below}

Applying a similar argument for the case $\mathcal{T} \tilde{U}(s) \leq \mathcal{T} \tilde{V}(s)$ results in

\begin{equation}
| \mathcal{T}^{\pi} \tilde{U} - \mathcal{T}^{\pi} \tilde{V} | < \gamma \Vert \tilde{U} - \tilde{V} \Vert + \epsilon .
\end{equation}

Since $\epsilon$ is an arbitrary positive number, we establish the result, i.e.,

\begin{equation}
| \mathcal{T}^{\pi} \tilde{U} - \mathcal{T}^{\pi} \tilde{V} | \leq \gamma \Vert \tilde{U} - \tilde{V} \Vert.
\end{equation}
\end{proof}



% \paragraph{Verification}

% \textbf{Introduce verification techniques: Discuss IBP, Dual Approach to Scalable Verification etc...}


% \paragraph{Adversarial training} involves perturbing the inputs...

% %Previous solutions?
% Previous work on verifiable/adversarial RL can be divided into a number of different categories

% \textbf{TODO - Add references}

% on examining the effects of adversarial attacks on an RL agent \cite{Huang2017}.

% \cite{Huang2017,Kos2017,Mandlekar2017,Pan2019,Pattanaik2018}. 

% Several methods have been proposed to find adversarial examples.
% \citet{goodfellow_explaining_2014} proposed one of the earliest method specific to $L_\infty$-bounded perturbations.
% It is known as the Fast Gradient Sign Method (FGSM):
% \begin{equation}
% x + \epsilon \text{sign} \left( \nabla_x L(x, y) \right)
% \end{equation}
% A more powerful adversary is the multi-step variant FGSM$^K$, which essentially performs $K$ PGD steps on the negative loss function~\citep{kurakin_adversarial_2016}:
% \begin{equation}
% x_{t+1} \gets \proj_{\mathcal{S}(x)} \left( x_t + \alpha \sign \left( \grad_{x_t} L(x_t, y) \right) \right)
% \end{equation}
% where $x_0$ is typically chosen at random within $S(x)$.
% Another popular method is from \cite{carlini_towards_2017} (C\&W) who extend the formulation of \cite{szegedy_intriguing_2013}.


% \section{Specification(s) for constraint satisfaction}


% This section provides examples of specifications for constraint satisfaction.

% \textbf{When perturbed, the mean (i.e.\ deterministic) action does not violate the constraint}
% I.e., even when perturbed, likely actions do not violate the constraint.
% \cosmo{The fact that we need to pick delta and an appropriate distance function seems a bit cumbersome right? It's fine if it is, I would just highlight it as a limitation.. Also, we may have constraints on actions, as in ACP, which might complicate things, but probably fine to ignore that for now.}
% % \begin{align*}
% % \forall s:&\,\, c(s, a_\mu + \delta) \leq  \beta \\
% % \text{s.t.}&\,\, a_\mu = \mathbb{E}[\pi(\cdot | s)]\\
% %     &\,\, |\delta| \leq \epsilon
% % \end{align*}

% \begin{align}
% \forall s:&\,\, c(s, \hat{a}) \leq  \beta \\
% \text{s.t.}&\,\, a_\mu = \mathbb{E}[\pi(\cdot | s)]\\
%     &\,\, \Vert \hat{a} - a_\mu \Vert \leq \delta
% \end{align}

% \danc{Sumanth mentioned that we can also handle state perturbations as well (assuming sensor noise). Further to Cosmin's point on smoothness on the transition dynamics, it seems that if we assume that transitions are smooth ($|s_t - s_{t+1}|$ is always small and bounded) then we can also use state perturbations as a proxy for using a dynamics model, and optimise over the next worst possible state! Which is great!}
% \danm{Agreed. Although, we may need models to simulate feasible next states. The issue we had in a previous work was that the next states, when perturbed by epsilon, may not actually be attainable states, which just adds noise to learning...}
% \danc{That is a fair point; in that case our resulting policies would be very conservative if they try to even minimize constraint violations for future infeasible states.}

% \section{The worst-case constraint violation}
% We can solve a constrained optimisation problem to find the maximum (i.e. worst-case) constraint violation $v^*$:

% % \begin{align}
% % v^* = \max_{a, \delta}\,\, & c(s, a + \delta) - \beta \\
% % \text{s.t.}&\,\, a \sim \bar{\pi}_{q}\\
% %     &\,\, |\delta| \leq \epsilon
% % \end{align}

% \begin{align}
% v^* = \max_{\hat{a}}& \,\, c(s, \hat{a}) - \beta \\
%     \text{s.t.}& \,\, \Vert \hat{a} - a_\mu \Vert \leq \delta\\
%     & \,\, a_\mu = \mathbb{E}[\pi(\cdot | s)]
% \end{align}



% Assuming we solved the problem above optimally, if $v^* \leq 0$ then we can \emph{certify} that the policy adheres to the specification for this state $s$.


% \section{Verifiable/Adversarial Constrained RL Objective}
% \danm{Do we want to try both action and state perturbations? Also, do we want to start with per time-step/episodic constraints?}
% Define the optimization problem as:

% \danc{At the moment this is saying that we are blending policies, one which tries to maximize reward, and the other which tries to minimize it (and both want to not violate immediate constraints). We discussed this a bit, it seems quite tricky, but we might be able to rephrase the adversarial policy as the one which tries to violate the most constraints, while still obtaining maximum reward.}

% \begin{eqnarray}
%     \max_{\pi \in \Pi} \min_{\bar{\pi} \in \Pi} \mathbb{E}^{\pi^{\text{mix}}_{N,\alpha}(\pi,\bar{\pi})}\biggl[\sum_t \gamma^t r(s_t,a_t) \biggr]&&\\
%     \text{s.t.} \forall s_t \in S, a_t \sim \pi^{\text{mix}}, \mathbb{E}\biggl[\mathbf{1}_{c(s_t,a_t)>\beta} \biggr] < \epsilon
% \end{eqnarray}

% \begin{eqnarray}
%     \max_{\pi \in \Pi} \min_{\bar{\pi} \in \Pi} \mathbb{E}^{\pi^{\text{mix}}_{N,\alpha}(\pi,\bar{\pi})}\biggl[\sum_t \gamma^t r(s_t,a_t) \biggr] + \min_{\bar{\pi}}\lambda (\mathbb{E}\biggl[\sum_{t} \gamma^t c(s_t,a_t) \biggr] - \beta)&&\\
%     \text{s.t.} \forall s_t \in S, a_t \sim \pi^{\text{mix}}, \mathbb{E}\biggl[\mathbf{1}_{c(s_t,a_t)>\beta} \biggr] < \epsilon
% \end{eqnarray}

% where $\pi^{\text{mix}}_{N,\alpha}(\pi,\bar{\pi})=(1-\alpha)*\pi + \alpha*\bar{\pi}$ is the mixture policy of the agent $\pi$ and the adversary $\bar{\pi}$.
% \cosmo{Any constraints on the adversary? Also how does this tie in with (3)-(5)?}

% \begin{eqnarray}
%     \max_{\pi \in \Pi} \min_{p\in P} \mathbb{E}^{P, \pi}\biggl[\sum_t \gamma^t r(s_t,a_t) \biggr]&&\\
%     \text{s.t.} \forall s_t \in S, a_t \sim \pi, \mathbb{E}\biggl[\mathbf{1}_{c(s_t,a_t)>\beta} \biggr] < \epsilon
% \end{eqnarray}

% where $p$ is an uncertainty set.

% \begin{eqnarray}
%     \max_{\pi \in \Pi} \min_{p\in P} \mathbb{E}^{P, \pi}\biggl[\sum_t \gamma^t r(s_t,a_t) \biggr]&&\\
%     \text{s.t.} \forall s_t \in S, a_t \sim \pi, \mathbb{E}\biggl[\sum_{t} \gamma^t c(s_t,a_t) \biggr] < \beta&&\\
% \end{eqnarray}

% \section{Contributions}


% \section{Adversarial/Verifiable MPO}
% \textbf{TODO - Apply this to constraints...}

% Previous work has not as yet identified the objective function that is being optimized when performing adversarial RL. In the following section, we show how the robust MDP objective can be modified to 


% % \begin{customthm}{1}
% % The robust \textbf{entropy-regularized} Bellman operator $\mathcal{T}^\pi_{\text{R-KL}}$ for a fixed policy $\pi$ is a contraction operator. Specifically:  $\forall U,V \in \mathbb{R}^{|S|}$ and $\gamma \in \left(0,1\right)$, we have, $\Vert \mathcal{T}^\pi_{\text{R-KL}}U - \mathcal{T}^\pi_{\text{R-KL}}V \Vert \leq \gamma \Vert U - V \Vert
% % $.

% % %For $U,V \in \mathbf{V}$, and $\gamma \in (0,1)$, the robust entropy-regularized Bellman operator $\mathcal{T}_{\text{R-KL}}$ for a deterministic policy $\pi$ is a $\gamma$-contraction in the sup norm:
% % %\nir{how about: The robust entropy-regularized Bellman operator $\mathcal{T}_{\text{R-KL}}$ is a contraction operator. Specifically: forall $U,V \in \mathbb{R}^{|s|}$ and $\gamma \in \left(0,1\right)$, we have}

% % \label{one}
% % %\label{thm:contraction}
% % \end{customthm}

% In order to account for model misspecification, in a previous project, we suggested to modify to policy evaluation step from:

% \begin{equation*}
%     \min_{\theta} \biggl(r_t + \gamma Q_{\hat{\theta}}^{\pi_{k}}(s_{t+1} \sim P(\cdot | s_t, a_t), a_{t+1}\sim \pi_{k}(\cdot \vert s_{t+1})) - Q_{\theta}^{\pi_{k}}(s_t, a_t) \biggr)^2,
% \end{equation*}

% to:

% \begin{equation*}
% \min_{\theta} \biggl(r_t + \gamma \color{red}\inf_{p \in \mathcal{P}(s_t, a_t)}\color{black} \biggl[Q_{\hat{\theta}}^{\pi_{k}}(s_{t+1} \sim p(\cdot | s_t, a_t), a_{t+1}\sim \pi_{k}( \cdot \vert s_{t+1}))  \biggr] - Q_{\theta}^{\pi_{k}}(s_t, a_t) \biggr)^2 \enspace ,
% \end{equation*}

% \begin{equation*}
% \min_{\theta} \biggl(r_t -\lambda c(s,a) + \gamma \color{red}\inf_{p \in \mathcal{P}(s_t, a_t)}\color{black} \biggl[Q_{\hat{\theta}}^{\pi_{k}}(s_{t+1} \sim p(\cdot | s_t, a_t), a_{t+1}\sim \pi_{k}( \cdot \vert s_{t+1}))  \biggr] - Q_{\theta}^{\pi_{k}}(s_t, a_t) \biggr)^2 \enspace ,
% \end{equation*}

% \begin{equation}
%     \min_{\theta} \Vert r(s,a) - \color{red}\inf_{p \in \mathcal{P}(s_t, a_t)}\color{black} L_{spec}(s',a,C) + \gamma Q(\theta, s, a) - Q(\theta, s, a) \Vert_2   
% \end{equation}

% \danc{In this case, we have access to a distribution over dynamics models, and we're saying that the next state will be the one resulting from our future action in the dynamics model with the worst action-value. Right?}  

% \danc{If so, we should connect this to violating constraints. I.e., select the next state in the inf term for the Q-function from the dynamics model where the agent would violate the constraint the most? (while learning a constraint function, immediate or action-value, for all possible dynamics models)}

% The above update requires knowledge of all transition models in the uncertainty set (or, at least, multiple actors in multiple perturbed environments, as we approximated it in a previous project). In order to alleviate this need, we propose to directly learning a worst-case value with respect to possible next-state realization, i.e.,

% \begin{equation*}
% \min_{\theta} \biggl(r_t + \gamma \color{blue}\inf_{s_{t+1} \in (\underline{s}_{t+1}, \overline{s}_{t+1})}\color{black} \biggl[Q_{\hat{\theta}}^{\pi_{k}}(s_{t+1}, a_{t+1}\sim \pi_{k}( \cdot \vert s_{t+1}))  \biggr] - Q_{\theta}^{\pi_{k}}(s_t, a_t) \biggr)^2 \enspace ,
% \end{equation*}

% \danc{Naive question incoming: how do we compute {$\color{blue}{s_{t+1} \in (\underline{s}_{t+1}, \overline{s}_{t+1})}$ }? Where do the two states come from (IBP)?}
% \cosmo{I actually had the same question :)}
% % \sven{For practical reasons, $a_{t+1}$ is sampled once for the nominal $s_{t+1}$, which is slightly different from what is written above:
% % \begin{equation*}
% % \min_{\theta} \biggl(r_t + \gamma \inf_{s \in (\underline{s}_{t+1}, \overline{s}_{t+1})} \biggl[Q_{\hat{\theta}}^{\pi_{k}}(s, a_{t+1}\sim \pi_{k}( \cdot \vert s_{t+1}))  \biggr] - Q_{\theta}^{\pi_{k}}(s_t, a_t) \biggr)^2 \enspace .
% % \end{equation*}}

% % \sven{The effect of the above is to create a more pessimistic version of the evaluation (as the action selected is not necessarily the most optimal action). We can remedy this issue in two ways. The first option is to maximize over the action to take at the next step:
% % \begin{equation*}
% % \min_{\theta} \biggl(r_t + \gamma \inf_{s \in (\underline{s}_{t+1}, \overline{s}_{t+1})} \sup_{a \in (\underline{a}_{t+1}, \overline{a}_{t+1})} \biggl[Q_{\hat{\theta}}^{\pi_{k}}(s, a)  \biggr] - Q_{\theta}^{\pi_{k}}(s_t, a_t) \biggr)^2 \enspace .
% % \end{equation*}

% % The other option is to use importance sampling:
% % \begin{equation*}
% % \min_{\theta} \biggl(r_t + \gamma \inf_{s \in (\underline{s}_{t+1}, \overline{s}_{t+1})} \biggl[\frac{\pi_{k}( a_{t+1} \vert s)}{\pi_{k}( a_{t+1} \vert s_{t+1})} Q_{\hat{\theta}}^{\pi_{k}}(s, a_{t+1}\sim \pi_{k}( \cdot \vert s_{t+1}))  \biggr] - Q_{\theta}^{\pi_{k}}(s_t, a_t) \biggr)^2 \enspace .
% % \end{equation*}
% % }

% % \sven{For simplicity, we can consider the set $(\underline{s}_{t+1}, \overline{s}_{t+1})$ to be $(s_{t+1} - \epsilon, s_{t+1} + \epsilon)$ where $\epsilon$ could be simple constant vector or a function of the state $s_{t+1}$.}

% % This raises two main questions:
% % \begin{enumerate}
% %     \item How can we transform the uncertainty set over transition models to a set over next-state realizations?
% %     \item How can we solve the inner $\inf$ optimization problem?
% % \end{enumerate}

% % We believe that for (1) can be treated in two ways: either simply tune a hyper-parameter that govern the next-state uncertainty set, or develop a theoretical result that connects the two uncertainty sets. As for (2), we plan on leveraging previous adversarial attacks results to approximate the solution.

% % \sven{For (1), I agree with the idea of a hyperparameter (at least initially) - this setting makes a lot of sense for sensor noise. Another option involves being able to simulate some perturbations and learn the mapping between the actual perturbation set $\mathcal{P}$. Yet another option is to have a curriculum that grows the set $(\underline{s}_{t+1}, \overline{s}_{t+1})$ reasonably as to still get good performance on the nominal unperturbed environment.}

% % \sven{For (2), the current suggestion is to use a single gradient step and reprojection onto $(\underline{s}_{t+1}, \overline{s}_{t+1})$: $s_{t+1}^{\star} = \textrm{Proj}\left(s_{t+1} + \alpha \nabla_{s} Q_{\hat{\theta}}^{\pi_{k}}(s, a_{t+1}\sim \pi_{k}( \cdot \vert s))\right)$. The reasoning is that while this will undoubtedly underestimate the worst-case, the function $Q$ is approximate by its very nature and the set $(\underline{s}_{t+1}, \overline{s}_{t+1})$ usually overestimates the true perturbation set. We can of course use multiple PGD steps with small $\alpha$ to get better solution.}

% \subsection{Solution methods}
% We should aim to get a closed-form solution to the worst-case violation optimisation problem.

% We can also use interval bound propagation to find an upper-bound (will be conservative).

% For example, we can define the actor loss as:

% \begin{equation}
%     L = L_{actor} + \alpha \cdot v^*
% \end{equation}
